LOss-Based SensiTivity rEgulaRization: towards deep sparse neural networks

LOBSTER (LOss-Based SensiTivity rEgulaRization) is a method for training neural networks having a sparse topology. Let the sensitivity of a network parameter be the variation of the loss function with respect to the variation of the parameter. Parameters with low sensitivity, i.e. having little impact on the loss when perturbed, are shrunk and then pruned to sparsify the network. Our method allows to train a network from scratch, i.e. without preliminary learning or rewinding. Experiments on multiple architectures and datasets show competitive compression ratios with minimal computational overhead.

==> 2_related_old.tex <==
\section{Related work}
\label{sec:sota}

It is well known that many ANNs, trained on some tasks, are typically over-parametrized~\cite{mhaskar2016deep, brutzkus2017sgd}. \attilio{In realta la prima reference dice solo che sotto certe condizioni una rete overparametrizzata llenata con SGD riesce comunque a generalizzare piuttosto che overfittare: questa affermazione non sara troppo forte ?.} \enzo{Agreed, frase riformulata}
Recently, it has been observed that the number of parameters effectively modified during the learning process is reduced: this suggests that all the others parameters can be removed from the learning process without affecting the performance~\cite{frankle2018lottery}.%\attilio{La parte finale di questa frase non é chiara.}
%AF: qui ho rifrasato il primo paragrafo della sez 2 di Han per dare una panoramica su come il finiding sopra possa essere sfruttato
A number of (orthogonal)\enzo{perche' orthogonal? non e' necessariamente vero} approaches have been put forward to leverage this finding.
For example, \cite{vanhoucke2011improving} quantizes the activation functions over a fixed number of bits.
\cite{denton2014exploiting} managed to exploit a low-rank approximation of the network parameters without incurring in too much penalty.
While the above approaches rely on quantization and compression to reduce the memory footprint of an ANN, this work relies instead on pruning connections between neurons.
While such approaches are orthogonal, pruning has in fact the beneficial side effect of improving a network generalization ability.\enzo{falso!}
For example, a large sparse architecture improves the network generalization ability in a number of different scenarios \cite{zhu2017prune}.\enzo{CAN improve... non e' un fatto, ma un positive side effect, tra l'altro non triviale da giustificare} \attilio{La citazione \cite{tartaglione2019post} starebeb bene qui visto che quel lavoro parla di generalizzazione.}

A number of different approaches to pruning exists.

A sound approach towards pruning parameters consists in exploiting a $l_2$ regularizer in a shrink-and-prune framework.
First, a standard $l_2$ regularization term is added to the cost function to minimize to shrink the magnitude of some parameters.
Next, parameters below a threshold are pinpointed to zero, learning a sparser topology,
Finally, the remaining parameters are fine-tuned and the whole procedure can be iterated \cite{han2015learning}.
Such approach is effective since regularization replaces unstable (ill-posed) problems with nearby and stable (well-posed) ones by introducing a prior on the parameters~\cite{Groetsch1993InverseProblems}.
However, as a drawback, this method requires a preliminary training to learn the initial connectivity via normal training, summing up to the training time.

Other approaches to introduce sparsity in ANNs attempt to rely on the optimal $l_0$ regularizer which, however, is a non-differentiable measure.
A recent work \cite{louizos2017learning} introduced a differentiable proxy measure to overcome this problem introducing, though, some relevant computational overhead. Having a similar overall approach, in another work a regularizer based on group lasso whose task is to cluster filters in convolutional layers is proposed \cite{wen2016structured}. Finally, such technique is not directly generalizeable to the bulky fully-connected layers, where most of the complexity (as number of parameters) lies.

%Early methods \cite{lecun1990optimal} rely on the Hessian of the loss function to prune connections, which entails however additional complexity to compute the second order derivatives.
%

Dropout-based approaches constitute another possibility to achieve sparsity. For example, \textit{Sparse VD} relies on variational dropout to promote sparsity \cite{molchanov2017variational}, providing also a Bayesian interpretation for Gaussian dropout.
Another dropout-based approach is \emph{Targeted Dropout} \cite{gomez2019targeted}: the training of the ANN model is self-reinforcing sparsity criterion by stochastically drop connections or units.

\emph{Soft Weight Sharing (SWS)} is another interesting approach~\cite{ullrich2017soft}: through such method, it is possible to effectively introduce redundancy in the parameters value, resulting in a lower number of parameters to be stored.\attilio{Questa citazione semra un teaser commerciale: non si capisce cosa faccia questo metodo da questo paragrafetto.}

Recently few-sample knowledge distillation (FSKD)~\cite{li2020few} has been proposed as a further approach that tries to overcome the need for large-scale training set transferring the knowledge from a large “teacher” network to a compact “student” network by matching certain statistics between them.

Other recent approaches mainly focus on the pruning of convolutional layers either leveraging on the artificial bee colony optimization algorithm (dubbed as ABCPruner)~\cite{lin2020channel} or using a small set of input to evaluate a saliency score and construct a sampling distribution~\cite{liebenwein2020provable}
\added{
%AF Qui citiamo il paper nips18 più che altro per chiarire in cosa consista la novelty rispetto a quel paper
The present work represents a significant improvement over our previous research \cite{tartaglione2018sensitivity}.
In our previous research, we introduced the sensitivity of a network parameter as a measure of how much the network output changes for small perturbations of the parameter.
%Attilio qui si assume che se il paper NIPS18 é stato preso , é perché era innovativo a quanto sotto
%(differently from what proposed in other works \cite{engelbrecht1996sensitivity,mrazova2011new,mrazova2012can}).
Next, a regularization strategy pushes low-sensitivity parameters towards zero, i.e. only parameters that do not affect the network output when perturbed are pruned.
%Such a technique, when compared with other state-of-the-art pruning approaches, introduces a reduced computational overhead.
However, such method requires the network to be already trained so to measure the variation of the network output when a parameter is perturbed, increasing the overall learning time.
In this work, we overcome this limitation introducing \emph{loss-based sensitivity}, which is also beneficial for generalization and further reduces the computation overhead. A detailed discussion between the differences from the two formulations follows in Sec.~\ref{sec::outsens}.

}
